Gromov-Thurston manifolds and anti-de Sitter geometry

We consider hyperbolic and anti-de Sitter (AdS) structures on $M\times (0,1)$, where $M$ is a $d$-dimensional Gromov-Thurston manifold. If $M$ has cone angles greater than $2\pi$, we show that there exists a "quasifuchsian" (globally hyperbolic maximal) AdS manifold such that the future boundary of the convex core is isometric to $M$. When $M$ has cone angles less than $2\pi$, there exists a hyperbolic end with boundary a concave pleated surface isometric to $M$. Moreover, in both cases, if $M$ is a Gromov-Thurston manifold with $2k$ pieces (as defined below), the moduli space of quasifuchsian AdS structures (resp. hyperbolic ends) satisfying this condition contains a submanifold of dimension $2k-3$. When $d=3$, the moduli space of quasifuchsian AdS (resp. hyperbolic) manifolds diffeomorphic to $M\times (0,1)$ contains a submanifold of dimension $2k-2$, and extends up to a "Fuchsian" manifold, that is, an AdS (resp. hyperbolic) warped product of a closed hyperbolic manifold by~$\R$. We use this construction of quasifuchsian AdS manifolds to obtain new compact quotients of $\O(2d,2)/\U(d,1)$. The construction uses an explicit correspondence between quasifuchsian $2d+1$-dimensional AdS manifolds and compact quotients of $\O(2d,2)/\U(d,1)$ which we interpret as the space of timelike geodesic Killing fields of $\AdS^{2d+1}$.

==> grothu6.bak.tex <==
\section{Initial singularities}
\label{sc:initial}
.\marginnote{JM va écrire une première version.}

\subsection{Dualities}

Before proving Theorems \ref{tm:initial-ads} and \ref{tm:initial-hyp}, we recall a basic notion of duality (or polarity) in $AdS^{d+1}$, or between $\HH^{d+1}$ and $dS^{d+1}$. A good description of the duality for hyperbolic polyhedra can be found in \cite{HR}, and an extension to other constant curvature pseudo-Riemannian spaces can be found e.g. in \cite{shu}. 

\subsubsection*{The duality between $\HH^{d+1}$ and $dS^{d+1}$}

Recall that the hyperbolic $d+1$-dimensional space can be defined as a quadric in the Minkowski space of dimension $d+2$, denoted here as $\R^{d+1,1}$. This Minkowski space is $\R^{d+2}$ equipped with the bilinear symmetric form:
$$ \langle x,y\rangle_{d+1,1} = -x_0^2 + \sum_{i=1}^{d+1} x_i^2~. $$
The hyperbolic space can then be defined as
$$ \HH^{d+1} = \{ x\in \R^{d+1,1}~|~\langle x,x\rangle_{d+1,1}=-1 \wedge x_0>0 \}~, $$
equipped with the induced metric.

In the same space, we can consider the de Sitter space, defined as
$$ dS^{d+1} = \{ x\in \R^{d+1,1}~|~\langle x,x\rangle_{d+1,1}=1 \}~, $$
again with the induced metric. It is a geodesically complete Lorentzian space of constant curvature $1$, simply connected if $d\geq 2$.

Let $x\in \HH^{d+1}$, and let $x^\perp$ be the hyperplane in $\R^{d=1,1}$ orthogonal to $x$. Since $x$ is time-like, its orthogonal $x^\perp$ is space-like, and its intersection with $dS^{d+1}$ is a totally geodesic, space-like hyperplane, which we denote by $x^*$. Conversely, any space-like hyperplane $H$ in $dS^{d+1}$ is the intersection of $dS^{d+1}$ with a hyperplane $\bar H$ of $\R^{d+1,1}$ containing $0$. This hyperplane $\bar H$ is orthogonal to a unique unit, future-oriented time-like vector, which we denote $H^*$. This construction provides a one-to-one correspondence between points in $\HH^{d+1}$ and (un-oriented) space-like totally geodesic hyperplanes in $dS^{d+1}$.

Similarly, given $y\in dS^{d+1}$, the intersection of $y^\perp\cap \HH^{d+1}$ is an {\em oriented} totally geodesic hyperplane in $\HH^{d+1}$, which we denote by $y^*$. And conversely, if $H\subset \HH^{d+1}$ is any oriented totally geodesic hyperplane, then it is the intersection with $\HH^{d+1}$ of an oriented hyperplane in $\R^{d+1,1}$ containing $0$. The oriented unit normal to this hyperplane is a point in $\dS^{d+1}$, which we denote by $H^*$. 

This duality relation has several important consequences.
\begin{itemize}
\item Two oriented hyperplanes $H,H'\subset \HH^{d+1}$ intersect if and only if the dual points $H^*, H'^*$ are connected by a space-like geodesic segment. The angle between $H$ and $H'$ is then the length of the segment connecting $H^*$ to $H'^*$.
\item The intersection angle between two hyperplanes $H, H'\subset dS^{d+1}$ is equal to the distance between the dual points $H^*, H'^*\subset \HH^{d+1}$.
  \item For all $x\in \HH^{d+1}$, $(x^*)^*=x$, and similarly for $y\in dS^{d+1}$.
  \marginnote{JM: to be completed with what is needed below.}
\end{itemize}
This duality relation extends to convex polyhedra (see \cite{HR}) and to smooth, strictly convex surfaces (see e.g. \cite{shu}). 


\subsubsection*{The duality between points and hyperplanes in $AdS^{d+1}$}

The $d+1$-dimensional anti-de Sitter space $AdS^{d+1}$ can be defined as a ``pseudo-sphere'' in the flat space $\R^{d,2}$ of signature $(2,d)$. Specifically, $\R^{d,2}$ can be defined as $\R^{d+2}$ equipped with the bilinear symmetric form
$$ \langle x,y\rangle_{d,2} = -x_0y_0 - x_1y_1 + \sum_{i=2}^{d+1} x_iy_i~, $$
and
$$ AdS^{d+1} = \{ x\in \R^{d,2}~|~ \langle x,y\rangle_{d,2} = -1\}~. $$
It is a geodesically complete Lorentzian space of constant curvature $-1$.

Let $x\in AdS^{d+1}$. Its orthogonal $x^\perp$ is an oriented hyperplane in $\R^{d,2}$ of signature $(1,d)$, which therefore intersects $AdS^{d+1}$ along a space-like totally geodesic oriented hyperplane, denoted by $x^*$. As above, the same construction works, conversely, to associate to any totally geodesic space-like oriented hyperplane a dual point.

This duality has the same properties as the duality between $\HH^{d+1}$ and $dS^{d+1}$.\marginnote{JM: more details?}\marginnote{JM: another reference?}

\subsection{Initial singularities of de Sitter spacetimes}

We briefly recall here some basic geometric properties of GHM de Sitter spacetimes, additional details and proofs can be found in \cite{kulkarni-pinkall,scannell}. 
We then briefly describe the duality between convex GHM de Sitter spacetimes and hyperbolic ends, and then outline how this duality leads to the proof of Theorem \ref{tm:initial-ds}.

Consider first a hyperbolic end $E$, diffeomorphic to $M\times \R$, where $M$ is a closed $d$-dimensional manifold. Then the boundary at infinity $\partial_\infty E$ of $E$ is diffeomorphic to $M$ and equipped with a flat conformal structure $c$. It is proved in \cite{kulkarni-pinkall} that $E$ is uniquely determined by $c$. Moreover, the concave pleated end of $E$ is determined by $c$. More specifically, the concave pleated end $\partial_0E$ of $E$ is equipped with a stratification in ideal polyhedra of varying dimensions between $1$ and $d$, while $(M,c)$ also has a natural stratification, with each point contained in the interior of the ``convex hull'' of the boundary of a unique maximal round ball. There is a natural map from $\partial_\infty E$ to $\partial_0E$, preserving the stratification, in the sense that each strata of the stratification of $\partial_\infty E$ is sent homeomorphically to a strata of $\partial_0E$ (but many strata of $\partial_\infty E$ can be sent to the same strata of $\partial_0E$). In fact, round balls in $\partial_\infty \HH^{d+1}$ are in one-to-one correspondence with oriented planes in $\HH^{d+1}$, and the strata of $(M,c)$ are in one-to-one correspondence with the support hyperplanes of $\partial_0M$. 

A similar construction is provided by Scannell \cite[Section 4]{scannell} for convex GHM de Sitter spacetimes. Namely, if $N$ is such a spacetime, diffeomorphic to $M\times \R$, where $M$ is again a closed $d$-dimensional manifold, then its future asymptotic boundary is equipped with a flat conformal structure $c$, and this flat conformal structure again uniquely determines the convex GHM structure on $N$. Convex GHM de Sitter structures on $N$ are therefore in one-to-one correspondence with hyperbolic ends diffeomorphic to $M\times \R$. 

The stratification of $(M,c)$ is directly related to the initial singularity of $N$. Round disks in $\partial_\infty \HH^{d+1}$ are in one-to-one correspondence with points in $dS^{d+1}$, and each stratum of $(M,c)$ determines a unique point in the initial singularity of $N$. The points that are obtained in this way are exactly those where the boundary of $M$ admits a space-like support hyperplane.\marginnote{JM: check, and add argument?}

Summing up the relations, each hyperbolic end structure on $M\times \R$ is determined uniquely by a flat conformal structure on $M$, which in turns determines a unique convex GHM de Sitter spacetime. Hyperbolic ends are therefore in one-to-one correspondence with convex GHM de Sitter spactimes. Moreover, each support hyperplane of $\partial_0M$ corresponds to a point to a point of $\partial M$ where it admits a space-like support plane, and conversely.

This correspondence is somewhat easier to visualize when the developing map $dev:(\tilde M,c)\to S^d$ is injective. Then
$$ E = (\HH^{d+1}\setminus CH(dev(\tilde M))/\rho(\pi_1M)~, $$
where $\rho:\pi_1M\to SO(d+1,1)$ is the holonomy representation of $(M,c)$, while $\tilde N$ can be identified with the intersection of the half-spaces containing $S^d$ and bounded by a hyperplane tangent to $S^d$ at a point of $\Lambda_\rho$, the limit set of $\rho$.

Suppose now that $E$ is a hyperbolic end such that $\partial_0E$ is folded, that is, it is the union of $2n$ $d$-dimensional polyhedra meeting along a $(d-1)$-dimensional leaves which share a $(d-2)$-dimensional manifold $S$. Let $N$ be the dual convex GHM de Sitter spacetime. The initial singularity of $N$ is then particularly simple:
\begin{itemize}
\item each $d$-dimensional polyhedron in $\partial_0E$ corresponds to a vertex of $\partial_0N$,\marginnote{JM: need to add this notation above.}
\item each $(d-1)$-dimensional intersection hypersurface in $\partial_0E$ corresponds to an edge of $\partial_0N$,
  \item the ``spine'' $S$ corresponds to a $2$-dimensional face of $\partial_0N$.
  \end{itemize}
  This proves Theorem \ref{tm:initial-ds}.

|example of a folded convex hypersurface in a hyperbolic end.]



%% structure of the universal cover of de Sitter GHM spacetimes
%% intersection of half-spaces bounded by tangent hyperplanes at infinity

%% the initial singularity is dual to the bending lamination

%% special case of convex folded hypersurfaces

%% the length of the edges of the initial singularity correspond to 

\subsection{Initial singularities of AdS spacetimes}

%% same as hyperbolic setting but the duality is with AdS

%% description of domain of dependence

%% special case when folded boundary

%% then boundary of dual contains dual tree.
